Uncertainty Quantification for Image-based Traffic Prediction across Cities

Despite the strong predictive performance of deep learning models for traffic prediction, their widespread deployment in real-world intelligent transportation systems has been restrained by a lack of interpretability. Uncertainty quantification (UQ) methods provide an approach to induce probabilistic reasoning, improve decision-making and enhance model deployment potential. To gain a comprehensive picture of the usefulness of existing UQ methods for traffic prediction and the relation between obtained uncertainties and city-wide traffic dynamics, we investigate their application to a large-scale image-based traffic dataset spanning multiple cities and time periods. We compare two epistemic and two aleatoric UQ methods on both temporal and spatio-temporal transfer tasks, and find that meaningful uncertainty estimates can be recovered. We further demonstrate how uncertainty estimates can be employed for unsupervised outlier detection on changes in city traffic dynamics. We find that our approach can capture both temporal and spatial effects on traffic behaviour in a representative case study for the city of Moscow. Our work presents a further step towards boosting uncertainty awareness in traffic prediction tasks, and aims to highlight the value contribution of UQ methods to a better understanding of city traffic dynamics.

==> chapters/4_sub_density.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/old/traffic_density.png}
    \caption{Relating uncertainty to traffic density. Ground truths (GT) and uncertainties (UQ) on logarithmic scale are plotted against a density proxy $\hat{k}$, sorted in ascending order of $\hat{k}$. We observe sudden shifts in specific sections of the density proxy, capturing changes in traffic dynamics. \todo{(need new plot)}}
    \label{fig:density}
\end{figure}

The fundamental traffic flow equation is $q = k \, \cdot \, v$, where $q$ is traffic flow, $k$ is traffic density and $v$ is average traffic speed. It can be used to compute the density as a ratio $q/v$ if flow and speed are known. The flow equation is satisfied only when the average traffic speed is computed by averaging over space, commonly referred to as space-mean speed $v_s$, in contrast to time-mean speed $v_t$ ~\citep{iitbombaylecture}. Formally, if we consider $n$ vehicles and vehicle $i$ travelling at speed $v_i$, we have $v_{s}=n/ \sum \frac{1}{v_{i}}$ and $v_{t}=\frac{1}{n} \sum_{i-1}^{n} v_{i}$. Three challenges exist in applying the flow equation to the \tfc dataset. Firstly, it is unclear how the averaging of speed and volume across car measurements in the data was done, and speed values might be a combination of $v_s$ and $v_t$. Secondly, values are represented as components along four intercardinal directions, thereby impeding a reconstruction of values in the directions of the actual road segments. %Specifically, a single pixel might correspond to multiple road segments with different directions of traffic, as is evident in~\autoref{fig:zoom_unc}. 
Thirdly, the data is normalised to the range $[0,255]$, so absolute values are difficult to interpret. In light of these challenges, our computed ratio $q/v$ does not necessarily yield the true traffic density but instead an approximation, which we refer to as \emph{density proxy} $\hat{k}$. In a similar approach, ~\citet{quasidensitypaper} remark that such quantities should be treated qualitatively and not in ``strict physical sense'', we therefore limit ourselves to such statements. 

To visualize how ground truths and uncertainties behave in relation to the density proxy, we plot their values on a logarithmic scale against the quantiles of $\hat{k}$ in ~\autoref{fig:density}, i.e. sorted in ascending order of $\hat{k}$. %In other words, all pixels are sorted in ascending order by their density proxy values and the corresponding speed and volume ground truths (GT) and uncertainties. The figure highlights the nuances in existing notions on the difficulty of traffic prediction. 
Deep learning-based traffic prediction has been observed to be more challenging for congested traffic conditions~\citep{kumar2021}. Higher traffic density typically implies higher levels of traffic congestion. \autoref{fig:density} shows that while the overall trend of uncertainty in speed and volume differ, the uncertainties in both quantities suddenly increase for specific density quantiles. Such regions of high uncertainty arise due to an underlying change in traffic dynamics. Specifically, the onset of high uncertainty regions lies in the second and third quartiles of density. It is compelling to link these observations to the scattered parts of the macroscopic fundamental diagram of traffic~\citep{zhang2020recent}, thereby hinting at a possible relationship between insights derived from traffic theory and those from a data-driven approach. Furthermore, $v_t$ and $v_s$ are related by the equation $v_{t}=v_{s}+\sigma^{2}_{v_s}/v_s$ ~\citep{iitbombaylecture}, which implies that when all vehicles travel at similar speeds, $v_s$ and $v_t$ are close to each other, and our density proxy is closer to the true traffic density since $q = k \cdot v_t = k \cdot v_s$. When the computed density proxy is close to the true density, the speed-density curve should be close to a straight line with negative slope \todo{(why?)}. Qualitatively, the insights from \autoref{fig:density} can be summarised as ``homogeneous traffic conditions typically exhibit low uncertainty''.




% The fundamental traffic flow equation is
% \begin{equation}
% \label{eq:fundamental-tr}
%     q = k \, \cdot \, v
% \end{equation}   
%  where $q$ is traffic flow, $k$ is traffic density and $v$ is average traffic speed. It can be used to compute the density if flow and speed are known. The flow equation is satisfied only when the average traffic speed is computed by averaging over space, commonly referred to as space-mean speed $v_s$, in contrast to time-mean speed $v_t$ ~\citep{iitbombaylecture}. Formally, if we consider $n$ vehicles, and vehicle $i$ travelling with speed $v_i$, we have:
%  % and is not satisfied when time-mean speed ($v_t$) is used in place of average traffic speed in the flow equation~\citep{iitbombaylecture}. Mathematically, if we consider $n$ vehicles, with each vehicle travelling at a speed $v_i$, the time-mean and space-mean speeds are given by ~\autoref{eq:timemeanspeed} and~\autoref{eq:spacemeanspeed}:
%  \begin{equation}
% %  \label{eq:timemeanspeed}
% v_{s}=\frac{n}{\sum \frac{1}{v_{i}}}, \ \ \ \  \ v_{t}=\frac{1}{n} \sum_{i-1}^{n} v_{i}
% \end{equation}

% % \begin{equation}
% % \label{eq:spacemeanspeed}
% % v_{s}=\frac{n}{\sum \frac{1}{v_{i}}}
% % \end{equation}

% It is unclear how the averaging of speed and volume channels in the \emph{Traffic4cast} dataset was done, and speed values might be a combination of $v_s$ and $v_t$. In addition, channel values are normalised to the range $[0,255]$, so absolute values are difficult to interpret.
% % Three specific challenges exist in applying the flow equation to the Traffic4cast data. First, it is not clear how the averaging of volume and speed channels of the Traffic4cast data was done. The speed channel in the data might be a combination of $v_s$ and $v_t$, thus might not satisfy the fundamental equation. Second, the speed and volume values are represented as components along four intercardinal directions; thereby impeding a full reconstruction of the actual speeds or volumes in the directions of the constituent road segment. Specifically, a single pixel might correspond to multiple road segments with different directions of traffic, as is evident in~\autoref{fig:zoom_unc}. Third, each channel in the data is normalised to the range $[0,255]$, so the absolute values are difficult to interpret; any interpretation should be ideally based on relative values. 
% In light of these challenges the ratio $\frac{q}{v}$ does not necessarily yield the true traffic density but instead an approximation, which we refer to as \emph{density proxy}. %Our choice is motivated by a similar approach by ~\citet{quasidensitypaper}, who compute this ratio without using space-mean speed and refer to it as ``quasi-density''. 
% We note that in a similar approach, ~\citet{quasidensitypaper} remark that such quantities should be treated qualitatively and not in ``strict physical sense''~\citep[p.~6]{quasidensitypaper}, we therefore limit ourselves %on the relation between uncertainty and traffic density 
% to such statements. 

% % To visualize how ground truths and uncertainties  behave in relation to this density proxy, we plot their values on a logarithmic scale against the quantiles of the density proxy variable in ~\autoref{fig:density}.
% %In other words, all pixels are sorted in ascending order by their density proxy values and the corresponding speed and volume ground truths (GT) and uncertainties 

% %One-to-one correspondence between each cell and its features (errors, GTs, UC) is maintained. 
% % The grids are sorted in ascending order according to the computed density-proxy for the grid.

  
%   %The insights from~\autoref{fig:density} make the existing notions of the difficulty in traffic prediction more nuanced. 
%   \autoref{fig:density} highlights the nuances in existing notions of the difficulty in traffic prediction.
%   Deep learning-based traffic prediction has been observed to be more challenging for congested traffic conditions~\citep{kumar2021applications}. Higher traffic density typically implies higher levels of traffic congestion. \autoref{fig:density} shows that while the overall trend of uncertainty in speed and volume differ, the uncertainties in both quantities suddenly increase for specific density quantiles. Such regions of high uncertainty arise due to an underlying change in traffic dynamics. Specifically, the onset of high uncertainty regions lies in the second and third quartiles of density. It is compelling to link these observations to the scattered parts of the macroscopic fundamental  diagram (MFD) of traffic~\citep{zhang2020recent}, thereby hinting at a possible relationship between these two notions, one from traffic theory and the other from a data-driven learning-based approach. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.6\columnwidth]{figures/traffic_density.png}
%     \caption{Relating uncertainty to traffic density. Ground truths (GT) and uncertainties (UQ) on  logarithmic scale are plotted against the density proxy per cell, sorted in ascending order of density proxy values. Median and max. for the density proxy are 0.012 and 0.293 respectively.}
%     \label{fig:density}
% \end{figure}
  
%   %By definition of the density proxy, we see increasing volume and decreasing speed with higher density. Higher traffic density typically implies higher congestion. Interestingly, the increase (and decrease) are not monotonous, but involve shifts at specific density proxy quantiles. 
% % While the mean PI widths (PI) are aligned well with the ground truth values and predictions, the uncertainties diverge slightly.
% %Future work could analyze these differences in more detail, e.g. with respect to the underlying traffic situation.

% % In the figure, we observe pockets of high uncertainty, high errors, and high absolute values at specific quantiles of density-proxy values. 

% % However, our inferences are entirely based on the density-proxy defined above and not the true traffic density. We believe future research into data-driven traffic forecasting should aim to improve prediction performance at <some quantile based metric> density values.

% % The density-proxy can be further dissected to unearth insights into the variations in the difficulty of modelling traffic based on the nature of traffic streams. We know that the  fundamental flow equation (\autoref{eq:fundamental-tr}) is valid only when $v=v_s$. However, $v_t$ and  $v_s$ can be shown to be related by~\autoref{eq:relbetween-vs-vt}~\citep{iitbombaylecture}, where $\sigma$ is the standard deviation of $v_i$'s.
% % \begin{equation}\label{eq:relbetween-vs-vt}
% % v_{t}=v_{s}+\frac{\sigma^{2}}{v_{s}}
% % \end{equation}
% % This equation implies that when all vehicles travel at similar speeds, the variance is close to $0$, $v_s$ and $v_t$ are close to each other, the fundamental flow equation holds irrespective of the averaging method used while computing raw speed, and our density-proxy is closer to true density. When the computed density-proxy is closer to the true density, the speed-density curve should  be closer to a straight line with a negative slope. Qualitatively, the insights from the~\autoref{fig:density} can be summarised as: ``homogeneous traffic conditions typically exhibit low UQs''.
% % \begin{equation}
% %     q=k \cdot v = k \cdot v_t = k \cdot v_s
% % \end{equation}


% % Hence, the speed or volume value from several grids might not have physical significance.

